WildDepth-v2: A Synchronized RGB--LiDAR--Radar Dataset and Benchmark for Metric Depth, Motion, and Tracking of Wildlife

Measuring animal distance and motion in metric units underpins abundance estimation, morphometrics, and movement ecology, yet monocular video lacks metric scale and wildlife datasets lack metric ground truth. We present WildDepth 2, extending the synchronized RGB-LiDAR WildDepth dataset in three directions. (i) Imaging radar: 37 RGB-LiDAR-4D-radar sequences (19,716 frames) with per-point Doppler velocity and a measured error budget, to our knowledge the first imaging-radar wildlife recordings. (ii) Benchmarking: a frozen, checksummed hidden test set for RGB-only distance estimation and RGB+sparse-LiDAR depth completion, evaluated separately on animal and background pixels. (iii) Motion and tracking: metric 3D trajectories obtained by lifting 2D tracks using LiDAR, radar, or monocular depth. Across 48,723 animal frames, object-level radar calibration improves monocular depth over scene-level LiDAR calibration without requiring LiDAR at inference (AbsRel 0.120 vs. 0.198), although animal-level LiDAR remains more accurate (0.052). Across 431 tracks, once-per-track radar scaling reduces 3D position error four-fold (2.20 to 0.58 m) and distance-sampling detection-function bias from -13% to -2%, matching once-per-track LiDAR calibration. Transferring radar Doppler onto LiDAR produces motion masks 3.7 times denser than radar alone at 72% precision, reduces moving-animal LiDAR accumulation error by 37%, and estimates radial speed (r = 0.60), albeit with approximately 50% underestimation.

==> tables/depth_table_generated.tex <==
\begin{table*}[ht]
\centering
\caption{Per-distance evaluation on the released WildDepth snippets. Uncalibrated (UC) vs LiDAR-calibrated (LC) camera-to-animal distance error. Lower is better for RMSE, AbsRel, SILog; higher is better for $\delta<1.25$.}
\label{tab:depth_comparison}
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{ll|cc|cc|cc|cc}
\toprule
\textbf{Metric} & \textbf{Model} & \multicolumn{2}{c|}{\textbf{5--10m}} & \multicolumn{2}{c|}{\textbf{10--20m}} & \multicolumn{2}{c|}{\textbf{20--30m}} & \multicolumn{2}{c}{\textbf{30--50m}} \\
 &  & UC & LC & UC & LC & UC & LC & UC & LC \\
\midrule
\multirow{7}{*}{RMSE (m)}
& DepthAnything & 6.10 & \textbf{1.61} & 6.73 & \textbf{3.29} & 9.93 & \textbf{4.35} & 15.86 & \textbf{10.44} \\
& DA-v2         & 3.75 & \textbf{2.06} & 11.90 & \textbf{5.81} & 12.84 & \textbf{6.07} & 21.16 & \textbf{13.88} \\
& DA-v3         & 8.79 & \textbf{2.01} & 8.79 & \textbf{3.23} & 11.21 & \textbf{4.27} & 16.28 & \textbf{8.98} \\
& DepthPro      & 14.75 & \textbf{4.09} & 9.91 & \textbf{4.19} & 10.66 & \textbf{5.51} & 14.87 & \textbf{11.96} \\
& DPT           & 14.27 & \textbf{4.45} & 13.77 & \textbf{5.45} & 12.42 & \textbf{5.11} & 14.21 & \textbf{10.52} \\
& MonoDepth2    & 18.79 & \textbf{7.36} & 14.82 & \textbf{6.75} & 14.40 & \textbf{7.15} & 18.72 & \textbf{12.33} \\
& MoGe2         & 6.68 & \textbf{2.07} & 8.41 & \textbf{4.36} & 11.78 & \textbf{4.17} & 23.17 & \textbf{8.08} \\
\midrule
\multirow{7}{*}{AbsRel}
& DepthAnything & 0.53 & \textbf{0.16} & 0.35 & \textbf{0.16} & 0.30 & \textbf{0.13} & 0.31 & \textbf{0.19} \\
& DA-v2         & 0.36 & \textbf{0.19} & 0.43 & \textbf{0.22} & 0.41 & \textbf{0.19} & 0.42 & \textbf{0.29} \\
& DA-v3         & 0.70 & \textbf{0.17} & 0.42 & \textbf{0.15} & 0.35 & \textbf{0.13} & 0.33 & \textbf{0.18} \\
& DepthPro      & 1.10 & \textbf{0.38} & 0.43 & \textbf{0.20} & 0.31 & \textbf{0.17} & 0.30 & \textbf{0.24} \\
& DPT           & 1.25 & \textbf{0.44} & 0.69 & \textbf{0.27} & 0.38 & \textbf{0.15} & 0.28 & \textbf{0.21} \\
& MonoDepth2    & 1.52 & \textbf{0.68} & 0.74 & \textbf{0.32} & 0.44 & \textbf{0.21} & 0.39 & \textbf{0.26} \\
& MoGe2         & 0.54 & \textbf{0.17} & 0.39 & \textbf{0.16} & 0.34 & \textbf{0.11} & 0.35 & \textbf{0.16} \\
\midrule
\multirow{7}{*}{SILog}
& DepthAnything & 0.72 & \textbf{0.17} & 0.67 & \textbf{0.24} & 0.73 & \textbf{0.20} & 0.81 & \textbf{0.37} \\
& DA-v2         & 0.73 & \textbf{0.23} & 1.02 & \textbf{0.26} & 1.07 & \textbf{0.20} & 1.13 & \textbf{0.38} \\
& DA-v3         & 0.68 & \textbf{0.19} & 0.77 & \textbf{0.22} & 0.83 & \textbf{0.19} & 0.83 & \textbf{0.28} \\
& DepthPro      & 0.73 & \textbf{0.25} & 0.68 & \textbf{0.28} & 0.89 & \textbf{0.25} & 0.74 & \textbf{0.33} \\
& DPT           & 0.67 & \textbf{0.26} & 0.63 & \textbf{0.26} & 0.65 & \textbf{0.21} & 0.69 & \textbf{0.30} \\
& MonoDepth2    & 0.79 & \textbf{0.39} & 0.96 & \textbf{0.33} & 0.89 & \textbf{0.29} & 1.01 & \textbf{0.42} \\
& MoGe2         & 0.59 & \textbf{0.16} & 0.78 & \textbf{0.23} & 0.86 & \textbf{0.18} & 0.87 & \textbf{0.24} \\
\midrule
\multirow{7}{*}{$\delta<1.25$}
& DepthAnything & 0.40 & \textbf{0.79} & 0.43 & \textbf{0.72} & 0.53 & \textbf{0.85} & 0.47 & \textbf{0.69} \\
& DA-v2         & 0.40 & \textbf{0.71} & 0.39 & \textbf{0.57} & 0.38 & \textbf{0.57} & 0.43 & \textbf{0.39} \\
& DA-v3         & 0.41 & \textbf{0.80} & 0.39 & \textbf{0.78} & 0.41 & \textbf{0.81} & 0.47 & \textbf{0.68} \\
& DepthPro      & 0.31 & \textbf{0.45} & 0.41 & \textbf{0.74} & 0.52 & \textbf{0.68} & 0.48 & \textbf{0.51} \\
& DPT           & 0.19 & \textbf{0.37} & 0.30 & \textbf{0.62} & 0.46 & \textbf{0.76} & 0.61 & \textbf{0.59} \\
& MonoDepth2    & 0.16 & \textbf{0.29} & 0.24 & \textbf{0.54} & 0.36 & \textbf{0.65} & 0.39 & \textbf{0.49} \\
& MoGe2         & 0.45 & \textbf{0.76} & 0.44 & \textbf{0.78} & 0.50 & \textbf{0.87} & 0.51 & \textbf{0.71} \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/tab_marigold.tex <==
% generated by scripts/make_tables.py -- do not edit by hand
\begin{tabular}{lcc}
\toprule
Protocol (AbsRel) & MoGe-2 & Marigold \\
\midrule
LC-scene (LiDAR) & 0.167 & 0.132 \\
LC-box held-out (LiDAR) & 0.060 & 0.056 \\
RC-box affine (radar) & 0.137 & 0.131 \\
RC-box leave-own-out (radar) & 0.257 & 0.194 \\
Hidden test Track A, LC & 0.094 & 0.252 \\
\bottomrule
\end{tabular}

